Pitfalls in Designing Zero-Effort Deauthentication: Opportunistic Human Observation Attacks

Deauthentication is an important component of any authentication system. The widespread use of computing devices in daily life has underscored the need for zero-effort deauthentication schemes. However, the quest for eliminating user effort may lead to hidden security flaws in the authentication schemes. As a case in point, we investigate a prominent zero-effort deauthentication scheme, called ZEBRA, which provides an interesting and a useful solution to a difficult problem as demonstrated in the original paper. We identify a subtle incorrect assumption in its adversary model that leads to a fundamental design flaw. We exploit this to break the scheme with a class of attacks that are much easier for a human to perform in a realistic adversary model, compared to the na\"ive attacks studied in the ZEBRA paper. For example, one of our main attacks, where the human attacker has to opportunistically mimic only the victim's keyboard typing activity at a nearby terminal, is significantly more successful compared to the na\"ive attack that requires mimicking keyboard and mouse activities as well as keyboard-mouse movements. Further, by understanding the design flaws in ZEBRA as cases of tainted input, we show that we can draw on well-understood design principles to improve ZEBRA's security.

==> chapters/5study_design.tex <==
\section{Attack Experiments}

%"Methodology"

%Nitesh + Prakash

\subsection{Study Design}

In this section, we present the design of our experiments to study the threat
of a human attacker impersonating a legitimate user by mimicking his/her activities
(keyboard, mouse and MKKM) based on audio/video. In particular, we study the 
audio KB-activity attack and video all-activity attack. 

%\subsection{Attacks}

%\subsubsection{Expert User Attack}

\subsection{Attacker Data Collection}

In our lab study, casual users served the role of the attackers. We recruited a
total of 20 users, 10 each for the audio KB-activity and video all-activity
attacks. The study participants were mostly students recruited by word of mouth.

In the study, the participants' goal was to reproduce victim's keyboard
activity based on audio clips, or all activities based on audiovisual clips (as
per the strategy outlined in Section \ref{sec:attack-strategy}). We collected only one
type of data, i.e., the input received by the OS through keyboard and mouse.
Before the study, participants were informed that everything they typed would
be logged and so were asked not to enter any sensitive information. We also
informed them that the purpose of the study was to study the ability of one
person to mimic the activity based on audio/video recordings. We purposely did
not disclose the true (security) purpose of the study so as not to bias the
participants' behavior in the experiment. The study was approved by our
University's IRB. The participation in the study was consent-based and strictly
voluntary.

%Two persons were involved in both of our experiments (audio KB-activity and
%video all-activity). First one was a user (serving as role of average attacker)
%and second was an experimenter (one of the researcher involved in the study)
%who assisted the user in the entire experiment.  The main job of experimenter
%was to instruct the user about the strategy to mimic the activity based on
%audio/video clip. 

The participants were subjected to a consent form and a demographic form before
the experiments. At the end of the experiments, their experience in mimicking
the activity based on the audio/video was recorded using a survey form.  The
survey contained 10 System Usable Scale (SUS) standard questions \cite{brooke1996a} and few task
specific questions, each with 5 possible responses (5-point Likert scale, where
1 represents strongly disagreement and 5 represents strongly agreement). The task specific questions contained few agree/disagree questionnaires like if they were distracted by the noise in the audio clips, if they could do better with audio-video combined, if they could mimic by direct observation of victim's activities etc.(you can see in Table \ref{table:study_score}) 
%% NS 2/2: should specify the additonal questions

 
 \medskip 
 \noindent \textbf{Audio KB-Activity Experiment:}\\ This experiment
 was designed to simulate our audio KB-activity attack, where the
 attacker attempts to impersonate the victim by mimicking victim's keyboard
 activity based on keyboard's audio sounds recorded by the audio listening
 device. 10 volunteering users participated in this experiment and, were
 %% NS 2/2: what does it mean by a small form? Shall we say what the form contained?
 asked to try to fill out a small web form while mimicking the KB-activity based
 on audio clip. We used a mobile device as a playback device and instructed
 participants to listen to the audio clips through earphones.  

Table \ref{table:study_demographics} (first column) shows the demographics of
our participants in this experiment. There were 70\% males and 30\% females.
These participants are composed of young educated individuals aged 18-35 years.
A majority of participants had Master's degree (80\%), from computer science and
engineering backgrounds. Most of them use computer frequently and
most of them were touch typist (70\%). None of the participants had hearing
problems.


\begin{table}[htbp]
		\caption{Demographics of participants in the audio KB-activity attack and video all-activity attack experiments} 
	\begin{center}{\scriptsize
		\begin{tabular}{|c|p{2cm}  |p{2cm}|}
			\hline
			& \textbf{Audio KB-activity} & \textbf{Video all-activity} \\
			\hline
				Participant Number (N=20) & 10 & 10 \\
			\hline
				\multicolumn{3}{c}{\bf Gender (\%)} \\
			\hline
				Male & 70 & 80 \\
				Female & 30 & 20 \\
			\hline
				\multicolumn{3}{c}{\bf Age (\%)} \\
			\hline
				18 - 24 & 10 & 20  \\
				25 - 35 & 90 & 80 \\
			\hline	
				\multicolumn{3}{c}{\bf Education (\%)} \\
			\hline
				Bachelor & 20 &  80 \\
				Masters & 80 & 20\\
			\hline
				\multicolumn{3}{c}{\bf Field of Study/Profession (\%)} \\
			\hline
				Computer Science &	40 & 70\\
				Engineering & 30 & 10\\
				Other & 30 & 20\\
			\hline	
				\multicolumn{3}{c}{\bf Computer Use (\%)} \\
			\hline
				Sometime 			& 20 & 0 \\
				Frequent 				& 80 & 100 \\
			
			\hline	
				\multicolumn{3}{c}{\bf Typing Style (\%)} \\
			\hline
				Touch Typist 			& 70 & 100\\
				Hand \& Peck Typist 		& 30 & 0 \\
			\hline	
		\end{tabular}
		
	}\end{center}


	\label{table:study_demographics}
\end{table} 

There were two phases in this experiment: (1)
``training'', and (2) ``testing''. It took approximately one hour to a
participant to complete this experiment. To prevent fatigue, we asked the
participants to take a short break after their training phase.

%% NS 2/2: random in what sense? Random from your pool of victim's recordings?
In the training phase, each of the participants was provided with four random
audio clips of the victim with varying difficulty level (collected previously
as described in Section \ref{victim-data}). They were asked to listen to each
of the audio clips carefully as per their need until they get sufficiently
confident that they could identify the keyboard sounds and mimic the keyboard
activities in the clip. Once they were confident, they were asked to fill out a
small web form repeatedly for five minutes by mimicking keyboard activities in
those clips. All of the recordings from this phase were considered as training
traces.
%of an average attacker.

In the testing phase, each of participants was provided with a different set of
four audio clips with varying difficulty level.  Unlike in testing phase, they
were not allowed to listen to any of these clips prior to the experiment. They
were asked to fill out the same web form repeatedly for five minutes based on
these fresh audio clips to the best of their abilities.  All of these
recordings were considered as testing traces and later used to analyze the performance 
of the attack.



\medskip
\noindent
\textbf{Video All-Activity Experiment:}\\
This experiment was designed to evaluate the video
all-activity attack, where the attacker attempts to impersonate the victim by
mimicking all the victim's activities based on the visual cues. For this
experiment, we asked a new set of 10 users to fill out the same small web (as in the previous experiment)
form by mimicking all the activities based on video clip. In this experiment,
half of the terminal's screen was used to play the video clip while another
half was used for the web form to be filled by the
participants. 

Table \ref{table:study_demographics} (second column) shows the demographics of
the 10 participants of our video all-activity attack experiment. Again, there were more males than females, at 80\% males vs 20\% females,
and all participants were young. They were also educated, mostly with Bachelor's degree
(80\%), and mostly from Computer science (70\%). All of the participants were
touch typist and use computers frequently in this case, in contrast to our
previous attack study. None of the participants had vision
problems.

Similar to the audio KB-activity experiment, this experiment comprised of
training and testing phases, and took approximately one hour for each
participant to complete. As earlier, participants of this experiment were asked
to take a short break after their training phase.

In the training phase, each of the participants was provided with four random
video clips with varying difficulty level (collected as described in Section
\ref{sec:victim-data}. Participants were asked to watch those video clips
carefully as per their need until they get sufficiently confident that they
could mimic the activities in the clip. Once they were confident, they were
asked to fill out the web form repeatedly for five minutes by mimicking
activities in the clip. 
%All of the recordings from this phase were considered
%as training traces of an average attacker. 
 
In the testing phase, each of participants was provided with another set of
four video clips. In contrast to testing phase, in this phase they were not
allowed to watch any of these clips prior to the experiment. They were asked to
fill out the same web form repeatedly for five minutes based on each of these
video clips to the best of their abilities. 
%All of these recordings were
%considered as testing traces of an average attacker.
 


\input{chapters/rta}



==> chapters/perception-results.tex <==
\subsection{User Perceptions}
\label{sec:perceptions}

Table \ref{table:study_score} depicts the user experience ratings for our two
attack experiments. For both experiments, the average SUS score was about 60.
Although these scores seem towards the lower end considering that industry
SUS averages end to hover in the 60--70 range
\cite{Lewis:1995:ICU:204770.204774}, they are still fairly reasonable. This is
because our study is an attack study not a traditional usability experiment.
We did not conduct our experiments to study the ease of use of software or to
study the usefulness of software, but rather to test the effectiveness of our
attack. These scores still indicate that the participants found that they could
perform the underlying tasks relatively easily and did not find them to be
complex. Intuitively, the all-activity experiment seems harder for the users
compared to the KB-activity experiment. However, comparing the average SUS
scores between the two experiments, using the Mann-Whitney U test, we did not
find any statistically significant difference ($p = 0.48$).

\begin{table}[h]
	\caption{User perceptions in our attack experiments}
	\begin{center}{\small
		\begin{tabular}{|c|p{2.5cm}|}
		
				\multicolumn{2}{c}{\bf SUS scores} \\
			\hline
			& Mean (Std. Dev.) \\&(max=100) \\
			\hline
			\
			Audio KB-activity & 59.75 (8.78) \\
			\hline
			
			Video all-activity & 58.75 (9.95)  \\
			\hline		

	\end{tabular}
	\vspace{20mm}
		\begin{tabular}{|p{5cm}|p{2cm}|}
							\multicolumn{2}{c}{\bf Audio KB-activity experiment specific questions} \\
			\hline
			& Mean (Std. Dev.) \\&(max=5)\\
			\hline
			\textit{Distracted by the noise in the audio clip}		& 2.9 (0.78)\\
			\hline
			\textit{Could mimic scrolling along with keyboard based on audio clip}	&	3.8 (0.6) \\
			\hline
			\textit{Could do better if video clip provided}		&	4.2 (0.94) \\
			\hline	
			\textit{Could mimic keyboard from surrounding sounds without any aid}	&	3.4 (0.65)  \\
			\hline
			\textit{Could do even better with further training}	&	3.8 (0.70) \\
			\hline
						\multicolumn{2}{c}{\bf Video all-activity experiment specific questions} \\
			\hline
			\textit{Distracted while switching back and forth between video and form}		& 3.4 (0.89)\\
			\hline
			\textit{Could do better if audio provided along with video}	&	3.8 (0.75) \\
			\hline
			\textit{Could mimic by watching one's activities without any aid}	&	3.6 (0.79) \\
			\hline
			\textit{Could do even better with further training}	&	3.9 (0.54)  \\
			\hline
				
			
			\end{tabular}
	}\end{center}
	\label{table:study_score}
\end{table}


Next, we considered participant responses to the task specific questions. We
see that the participants were not distracted by the noise in the audio clips
in the audio all-activity attack experiment. They seemed only slightly
distracted while switching back and forth between the video and the form in the
video all-activity attack experiment. The results also show that the
participants of the audio KB-activity attack were towards agreement that they
could distinguish the scrolling sound along with keyboard sound and could even
mimic them based on the audio clip. This suggests that the audio all-activity
attack might also be effective.  Moreover, the results of both experiments show
that the participants could perform better if both audio and video of victim's
activities were provided. This seems to suggest that audio-video KB-activity
and audio-video all-activity attacks could be more effective than the attacks
we studied.  Finally, and perhaps most interestingly, the participants felt
that they can perform better at the tasks with further training (we recall that
our participants were only trained with two 5-minute samples in each
experiment).  This underscores that the performance of the attacks may improve
significantly since the attacker can pursue offline training for hours before
attempting to attack the system. By contrast, the attack experiments presented
by Mare et al.\ \cite{mare2014zebra} did not consider this important element
which may have contributed to the poor performance of their attacks. 

%They were towards agreeing that with more
%training, they could do better. They were more or less neutral on if they could
%mimic KB-activity based on surrounding sounds without any aid. They were also
%more or less neutral on if they could mimic by observing the victim's
%activities directly.



		


==> chapters/rta.tex <==

\subsubsection{Real-time Attack}

